Dynamic Resource Allocation: Algorithmic Design Principles and Spectrum of Achievable Performances

Dynamic resource allocation problems are ubiquitous, arising in inventory management, order fulfillment, online advertising, and other applications. We initially focus on one of the simplest models of online resource allocation: the multisecretary problem. In the multisecretary problem, a decision maker sequentially hires up to $B$ out of $T$ candidates, and candidate ability values are drawn i.i.d. from a distribution $F$ on $[0,1]$. First, we investigate fundamental limits on performance as a function of the value distribution under consideration. We quantify performance in terms of regret, defined as the additive loss relative to the best performance achievable in hindsight. We present a novel fundamental regret lower bound scaling of $\Omega(T^{1/2 - 1/2(1 + \beta)})$ for distributions with gaps in their support, with $\beta$ quantifying the mass accumulation of types (values) around these gaps. This lower bound contrasts with the constant and logarithmic regret guarantees shown to be achievable in prior work, under specific assumptions on the value distribution. Second, we introduce a novel algorithmic principle, Conservativeness with respect to Gaps (CwG), which yields near-optimal performance with regret scaling of $\tilde{O}(T^{1/2 - 1/2(1 + \beta)})$ for any distribution in a class parameterized by the mass accumulation parameter $\beta$. We then turn to operationalizing the CwG principle across dynamic resource allocation problems. We study a general and practical algorithm, Repeatedly Act using Multiple Simulations (RAMS), which simulates possible futures to estimate a hindsight-based approximation of the value-to-go function. We establish that this algorithm inherits theoretical performance guarantees of algorithms tailored to the distribution of resource requests, including our CwG-based algorithm, and find that it outperforms them in numerical experiments.

==> latexmkrc <==
# This shows how to use the xr package with latexmk.
# John Collins 2023-03-29
#
# The xr package ("a system for eXternal References") is used by a document
# to make references to sections, equations, etc in other external
# documents. 
# The definitions in this file enable latexmk to apply latexmk to
# automatically update an external document whenever its .tex file changes,
# so that the references in the main document stay up to date.

# Notes:
#    1. This version is defined to put the files from the compilations of
#       the external documents into a defined subdirectory, to segregate
#       potentially many generated files from the main document
#       directories. 
#    2. But for latexmk's custom dependency mechanism to be used, as here,
#       the aux file from compilation of a subdocument must be generated in
#       the same directory as the corresponding source .tex file.  So the
#       .aux file is copied.
#    3. It is assumed that the external documents are to be compiled by
#       pdflatex.  This can be changed, of course, by changing the '-pdf'
#       option given to the invoked latexmk to whatever is needed.
#    4. An ideal implementation would also ensure that recompilation of an
#       external document also happens whenever any of its other source
#       files changes.  But this is not done in the present version, and
#       would probably entail either the use of internal latexmk variables
#       or extra enhancements to latexmk.
#    5. The code uses subroutines copy and fileparse that are loaded by
#       latexmk from the Perl packages File::Copy and File::Basename.
#    6. It also uses some not-yet-documented features of latexmk: an array
#       variable @file_not_found and subroutines popd, pushd, and
#       rdb_add_generated. 


#--------------------
# Configurable choices for compilation of external documents

# Subdirectory for output files from compilation of external documents:
$sub_doc_output = 'output-subdoc';

# Options to supply to latexmk for compilation of external documents:
@sub_doc_options = ();

push @sub_doc_options, '-pdf'; # Use pdflatex for compilation of external documents.
# Replace '-pdf' by '-pdfdvi', 'pdfxe', or 'pdflua' if needed.

#--------------------

# Add a pattern for xr's log-file message about missing files to latexmk's
# list.  Latexmk's variable @file_not_found is not yet documented.
# This line isn't necessary for v. 4.80 or later of latexmk.
push @file_not_found, '^No file\\s*(.+)\s*$';

add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
sub makeexternaldocument {
    if ( $root_filename ne $_[0] )  {
        my ($base_name, $path) = fileparse( $_[0] );
        pushd $path;
        my $return = system "latexmk",
                            @sub_doc_options,
                            "-aux-directory=$sub_doc_output",
                            "-output-directory=$sub_doc_output",
                            $base_name;
        if ( ($sub_doc_output ne ' ') && ($sub_doc_output ne '.') ) {
               # In this case, .aux file generated by pdflatex isn't in same
               # directory as the .tex file.
               # Therefore:
               # 1. Actual generated aux file must be listed as produced by this
               #    rule, so that latexmk deals with dependencies correctly.
               #    (Problem to overcome: If $sub_dir_output is same as $aux_dir
               #    for the main document, xr may read the .aux file in the
               #    aux_dir rather than the one the cus dep is assumed by latexmk
               #    to produce, which is in the same directory as the .tex source
               #    file for this custom dependency.)
               #    Use not-yet-documented latexmk subroutine rdb_add_generated
               #    to do this:
               # 2. A copy of the .aux file must be in same directory as .tex file
               #    to satisfy latexmk's definition of a custom dependency.
             rdb_add_generated( "$sub_doc_output/$base_name.aux" );
             copy "$sub_doc_output/$base_name.aux", ".";
        }
        popd;
        return $return;
   }
}
